Choosing The Best Interpolation Data in Images with Noise

We introduce and discuss shape based models for finding the best interpolation data in compression of images with noise. The aim is to reconstruct missing regions by means of minimizing data fitting term in the $L^2$-norm between the images and their reconstructed counterparts. We analyse the proposed models in the framework of the $\Gamma$-convergence from two different points of view. First, we consider a continuous stationary PDE model and get pointwise information on the "relevance" of each pixel by a topological asymptotic method. Second, we introduce a finite dimensional setting into the continuous model based on fat pixels (balls with positive radius), and we study by $\Gamma$-convergence the asymptotics when the radius vanishes. We extend the method to time-dependent based reconstruction and discuss several strategies for choosing the interpolation data within masks that might be improved over the iterations. Numerical computations are presented that confirm the usefulness of our theoretical findings for stationary and non-stationary PDE-based image compression.

==> tex_parts/section04.tex <==
\section{Gaussian Noise Model}
\label{sec:gaussian-noise}

As said previously, we consider that the input signal is affected by Gaussian noise. We consider the probability space $(\Omega,\mathcal{B}(\R),\mathbb{P})$. In this section, we assimilate the image $f$ as a random vector. We consider a random vector $G$ such that each $G_i$ follows a normal distribution with $F_i$ as mean and $\sigma$ standard deviation and all $G_i$ are independent. Then, each $G_i$ satisfies 

\[ \mathbb{P}(G_i\ |\ F_i) = \frac{1}{\sigma\sqrt{2\pi}} e^{-\frac{1}{2\sigma^2}(g_i-f_i)^2}. \]

Since every variable is independent, we have 

\[ \mathbb{P}(G\ |\ F) = \prod_{i=0}^N \mathbb{P}(G_i\ |\ F_i) = \frac{1}{\sigma\sqrt{2\pi}} e^{-\frac{1}{2\sigma^2}\sum_{i=0}^N(g_i-f_i)^2} = \frac{1}{\sigma\sqrt{2\pi}} e^{-\frac{1}{2\sigma^2} \|g-f\|_2^2}. \]

For denoising purpose, we generally use the ``maximum-a-posteriori estimate'' \cite{Wetzstein2017EE3, 6737048} of $f=(f_i)_{i=1}^N$ in $\R^N$ for a given $g$ in $\R^N$, that is

\[ \max_{f\in\R^N} \mathbb{P}(F = f\ |\ G = g), \]

or equivalently 

\[ \max_{f\in\R^N} \ln\mathbb{P}(F\ |\ G). \]

By using Bayes formula, we get  

\begin{align*}
    \max_{f\in\R^N} \ln\mathbb{P}(F\ |\ G) &= \max_{f\in\R^N} \ln\frac{\mathbb{P}(F)\mathbb{P}(G\ |\ F)}{\mathbb{P}(G)} \\
    %
     &= \max_{f\in\R^N} \ln\mathbb{P}(F) + \ln\mathbb{P}(G\ |\ F) - \ln\mathbb{P}(G).
\end{align*}

Since $\mathbb{P}(G)$ does not depends on $f$, we obtain

\[ \max_{f\in\R^N} \mathbb{P}(F\ |\ G) \Leftrightarrow \min_{f\in\R^N} \frac{1}{2\sigma^2} \|g-f\|_2^2 + \ln\mathbb{P}(F). \]

We call $\mathbb{P}(F)$ the prior on images. If we consider a uniform prior on images with normalized intensity values, which is $\mathbb{P}(F_i=f_i) = 1$ if $0\leq f_i \leq 1$ and $0$ otherwise, we have that the maximum-a-posteriori estimate of $F$ is equivalent to 

\[ \min_{f\in [0,1]^N} \|g-f\|_2^2. \]

This result shows us that, minimizing the $L^2$-error is equivalent as removing Gaussian noise. As a result, we focus our study on the $L^2$-error in the sequel.
